Unit Cell Phase-Frequency Profile Optimization in RIS-Assisted Wide-Band OFDM Systems

The reflection characteristics of a reconfigurable intelligent surface (RIS) depend on the phase response of the constituent unit cells, which is necessarily frequency dependent. This paper investigates the role of an RIS constituting unit cells with different phase-frequency profiles in a wide-band orthogonal frequency division multiplexing (OFDM) system to improve the achievable rate. We first propose a mathematical model for the phase-frequency relationship parametrized by the phase-frequency profile's slope and phase-shift corresponding to a realizable resonant RIS unit cell. Then, modelling each RIS element with $b$ control bits, we propose a method for selecting the parameter pairs to obtain a set of $2^b$ phase-frequency profiles. The proposed method yields an RIS design that outperforms existing designs over a wide range of user locations in a single-input, single-output (SISO) OFDM system. We then propose a low-complexity optimization algorithm to maximize the data rate through the joint optimization of (a) power allocations across the sub-carriers and (b) phase-frequency profile for each RIS unit cell from the available set. The analysis is then extended to a multi-user multiple-input single-output (MISO) OFDM scenario. Numerical results show an improvement in the coverage and achievable rates under the proposed framework as compared to single-slope phase-frequency profiles.

==> Figures/RISConfiguration/Dog.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
grid=major,
width=4.521in,
height=3.55in,
scale only axis,
xmin=2.4,
xmax=2.6,
xtick={2.4,2.45,2.5,2.55,2.6},
xticklabels={{$2.4$},{$2.45$},{$2.5$},{$2.55$},{$2.6$}},
xlabel style={at={(axis cs:2.5,-3.45)},anchor=north},
xlabel={$f$(GHz)},
separate axis lines,
every outer y axis line/.append style={mycolor1},
every y tick label/.append style={font=\color{mycolor1}},
every y tick/.append style={mycolor1},
ymin=-3.15,
ymax=3.15,
ytick={-3.14159265358979,-1.5707963267949,0,1.5707963267949,3.14159265358979},
yticklabels={{$-\pi$},{$-\frac{\pi }{2}$},{$0$},{$\frac{\pi}{2}$},{$\pi$}},
ylabel style={font=\color{mycolor1},at={(axis cs:2.397,0)},anchor=north},
ylabel={$\phi$},
axis background/.style={fill=white},
yticklabel pos=left,
xmajorgrids,
ymajorgrids,
legend style={{at =  (axis cs:2.4,-3.15)}, nodes={scale=0.75, transform shape}, anchor=south west, legend cell align=left, align=left, draw=black}
]
\addplot [color=mycolor1, dotted, line width=1.5pt]
  table[row sep=crcr]{%
2.4	2.89497281457813\\
2.403	2.8897116348121\\
2.406	2.88415859598954\\
2.409	2.87828840660036\\
2.412	2.87207277736404\\
2.415	2.86547996538284\\
2.418	2.85847423288571\\
2.421	2.85101520138453\\
2.424	2.84305707700706\\
2.427	2.83454771617106\\
2.43	2.82542749208431\\
2.433	2.81562791104753\\
2.436	2.80506991214526\\
2.439	2.79366176313738\\
2.442	2.7812964370531\\
2.445	2.7678483150124\\
2.448	2.75316900654863\\
2.451	2.73708200232557\\
2.454	2.7193757652904\\
2.457	2.69979470916709\\
2.46	2.6780272832689\\
2.463	2.65369004135382\\
2.466	2.62630605822456\\
2.469	2.59527527166193\\
2.472	2.55983310658387\\
2.475	2.51899181477634\\
2.478	2.47145589305936\\
2.481	2.41549799763359\\
2.484	2.34877380546189\\
2.487	2.26804167243623\\
2.49	2.16873424158198\\
2.493	2.04430664657317\\
2.496	1.88528082709848\\
2.499	1.6780134710457\\
2.502	1.40377878006864\\
2.505	1.04068763892217\\
2.508	0.574965421114847\\
2.511	0.0266465263349865\\
2.514	-0.534927895101642\\
2.517	-1.03060305053195\\
2.52	-1.42480558740385\\
2.523	-1.72410068243957\\
2.526	-1.94976141093636\\
2.529	-2.12195970658146\\
2.532	-2.25586146129132\\
2.535	-2.36209034454207\\
2.538	-2.44797730376978\\
2.541	-2.51861650462472\\
2.544	-2.5776034574866\\
2.547	-2.62752325583447\\
2.55	-2.67026985909209\\
2.553	-2.70725617299056\\
2.556	-2.73955416278496\\
2.559	-2.76798985427219\\
2.562	-2.79320887061872\\
2.565	-2.81572242176726\\
2.568	-2.83594010946891\\
2.571	-2.85419369214981\\
2.574	-2.87075455172046\\
2.577	-2.88584670567689\\
2.58	-2.89965662293136\\
2.583	-2.91234071529783\\
2.586	-2.92403111730613\\
2.589	-2.93484019060499\\
2.592	-2.94486406750606\\
2.595	-2.9541854631532\\
2.598	-2.96287592559959\\
2.601	-2.970997649973\\
};
\addlegendentry{$C_{d,1}$ = 0.6, $C_{d,2} = 3$ (pF)}

\addplot [color=mycolor1, dashed, line width=1.5pt]
  table[row sep=crcr]{%
2.4	2.87486901442694\\
2.403	2.86837076962763\\
2.406	2.86146669974259\\
2.409	2.85411722655262\\
2.412	2.8462774778499\\
2.415	2.83789637643655\\
2.418	2.82891553541575\\
2.421	2.81926791027399\\
2.424	2.8088761433568\\
2.427	2.79765051624483\\
2.43	2.78548639816782\\
2.433	2.77226104093265\\
2.436	2.75782951845565\\
2.439	2.74201953527593\\
2.442	2.72462472343841\\
2.445	2.70539589566157\\
2.448	2.68402950117578\\
2.451	2.66015220197282\\
2.454	2.63329999232663\\
2.457	2.60288952769279\\
2.46	2.56817815374971\\
2.463	2.52820727296928\\
2.466	2.48172072317814\\
2.469	2.4270450569579\\
2.472	2.3619108596065\\
2.475	2.28318185737486\\
2.478	2.18643978235233\\
2.481	2.06534887710798\\
2.484	1.91071162421722\\
2.487	1.70920963490408\\
2.49	1.44231071213014\\
2.493	1.08759820370581\\
2.496	0.628852111091746\\
2.499	0.0814781171403513\\
2.502	-0.487641881438627\\
2.505	-0.995408426677046\\
2.508	-1.40083154579095\\
2.511	-1.70839883032505\\
2.514	-1.93963526307703\\
2.517	-2.1155024233962\\
2.52	-2.25182761247978\\
2.523	-2.35968002303391\\
2.526	-2.44667274788337\\
2.529	-2.518076831344\\
2.532	-2.57759976725076\\
2.535	-2.62789880302632\\
2.538	-2.67091532856306\\
2.541	-2.70809406118503\\
2.544	-2.74052871464284\\
2.547	-2.76906044990569\\
2.55	-2.79434559547213\\
2.553	-2.81690304569387\\
2.556	-2.8371479920571\\
2.559	-2.85541630785377\\
2.562	-2.87198243666991\\
2.565	-2.88707269583581\\
2.568	-2.900875296461\\
2.571	-2.91354797995626\\
2.574	-2.92522390213257\\
2.577	-2.93601621344389\\
2.58	-2.94602165826763\\
2.583	-2.95532342843637\\
2.586	-2.96399344428842\\
2.589	-2.97209419222126\\
2.592	-2.97968021571948\\
2.595	-2.98679933344147\\
2.598	-2.99349364069324\\
2.601	-2.99980033776552\\
};
\addlegendentry{$C_{d,1}$ = 0.5, $C_{d,2} = 3$ (pF)}

\addplot [color=mycolor1, line width=1.5pt]
  table[row sep=crcr]{%
2.4	2.85328802256024\\
2.403	2.84531118029712\\
2.406	2.83677601768934\\
2.409	2.82762148326332\\
2.412	2.81777734334256\\
2.415	2.80716240028772\\
2.418	2.7956822823087\\
2.421	2.78322668070005\\
2.424	2.7696658678772\\
2.427	2.7548462702316\\
2.43	2.73858478588305\\
2.433	2.72066141721343\\
2.436	2.70080961366992\\
2.439	2.67870346372684\\
2.442	2.65394049177101\\
2.445	2.62601823483364\\
2.448	2.59430187955281\\
2.451	2.5579788401868\\
2.454	2.51599393532436\\
2.457	2.46695524226624\\
2.46	2.40899489583333\\
2.463	2.33955966359676\\
2.466	2.25509114116599\\
2.469	2.15053330667591\\
2.472	2.0185799251653\\
2.475	1.84857728613755\\
2.478	1.62516824756162\\
2.481	1.32759051280293\\
2.484	0.93321699788942\\
2.487	0.433462266350135\\
2.49	-0.136742262239498\\
2.493	-0.695103924957325\\
2.496	-1.16832285849271\\
2.499	-1.53545621458536\\
2.502	-1.81132388362565\\
2.505	-2.01892743901747\\
2.508	-2.17767692823538\\
2.511	-2.30157029118859\\
2.514	-2.40025746478025\\
2.517	-2.48036338255508\\
2.52	-2.54649074767505\\
2.523	-2.60189499867696\\
2.526	-2.64892399330607\\
2.529	-2.68930387345198\\
2.532	-2.72432691602355\\
2.535	-2.75497694570242\\
2.538	-2.78201455323174\\
2.541	-2.80603604516929\\
2.544	-2.82751493500397\\
2.547	-2.8468316302651\\
2.55	-2.86429500389097\\
2.553	-2.88015829546192\\
2.556	-2.89463099038428\\
2.559	-2.90788780511971\\
2.562	-2.920075562176\\
2.565	-2.93131850702221\\
2.568	-2.94172246113148\\
2.571	-2.95137809610171\\
2.574	-2.96036353725011\\
2.577	-2.96874645077022\\
2.58	-2.97658572956352\\
2.583	-2.98393286457815\\
2.586	-2.99083306775247\\
2.589	-2.99732619731288\\
2.592	-3.00344752470632\\
2.595	-3.00922837380394\\
2.598	-3.01469665644393\\
2.601	-3.01987732335037\\
};
\addlegendentry{$C_{d,1}$ = 0.4, $C_{d,2} = 3$ (pF)}
\end{axis}

\begin{axis}[%
width=4.521in,
height=3.55in,
scale only axis,
xmin=2.4,
xmax=2.6,
axis x line=none,
every outer y axis line/.append style={mycolor2},
every y tick label/.append style={font=\color{mycolor2}},
every y tick/.append style={mycolor2},
ymin=0.82,
ymax=1,
ytick={1,0.955,0.91,0.865,0.82},
yticklabels={{$1$},{$0.95$},{$0.9$},{$0.86$},{$0.82$}},
axis y line*=right,
ylabel style={font=\color{mycolor2},at={(axis cs:2.645,0.91)},anchor=north},
ylabel={$|\Gamma|$},
yticklabel pos=right,
legend style={at={(0.578,0.728)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor2, dotted, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
2.4	0.998669907764808\\
2.403	0.998591087000966\\
2.406	0.99850532869124\\
2.409	0.998411814819071\\
2.412	0.998309604425394\\
2.415	0.998197610892907\\
2.418	0.998074574209511\\
2.421	0.997939026909303\\
2.424	0.997789252000531\\
2.427	0.997623230666957\\
2.43	0.997438576822683\\
2.433	0.997232454635884\\
2.436	0.997001473808602\\
2.439	0.996741555552578\\
2.442	0.996447759604988\\
2.445	0.996114058941845\\
2.448	0.995733043550069\\
2.451	0.995295526920264\\
2.454	0.99479001758957\\
2.457	0.994202001165073\\
2.46	0.993512952722285\\
2.463	0.992698960355432\\
2.466	0.991728779920238\\
2.469	0.990561045481219\\
2.472	0.98914020801791\\
2.475	0.987390531278635\\
2.478	0.985207082448808\\
2.481	0.98244203489269\\
2.484	0.978883657672079\\
2.487	0.97422410294568\\
2.49	0.968011070557241\\
2.493	0.959580449390104\\
2.496	0.947983067321949\\
2.499	0.931985333224982\\
2.502	0.910437416471956\\
2.505	0.883764069871939\\
2.508	0.857291341435832\\
2.511	0.842995520090733\\
2.514	0.850325395812779\\
2.517	0.873985970708668\\
2.52	0.901242057637462\\
2.523	0.924501390508494\\
2.526	0.942157798850844\\
2.529	0.955056268478982\\
2.532	0.964445255142285\\
2.535	0.971355998378293\\
2.538	0.976527949419985\\
2.541	0.980469018602223\\
2.544	0.983525532929819\\
2.547	0.985935416020985\\
2.55	0.987864377723585\\
2.553	0.989429701725416\\
2.556	0.990715784017323\\
2.559	0.991784345568644\\
2.562	0.992681224282966\\
2.565	0.99344095681907\\
2.568	0.994089916467318\\
2.571	0.99464849483819\\
2.574	0.99513264117081\\
2.577	0.995554963765639\\
2.58	0.995925528660852\\
2.583	0.996252446085834\\
2.586	0.996542306192513\\
2.589	0.99680050640502\\
2.592	0.997031499913226\\
2.595	0.997238986152806\\
2.598	0.997426058157121\\
2.601	0.997595317529701\\
};
\addplot [color=mycolor2, dashed, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
2.4	0.998351652686395\\
2.403	0.998242936386042\\
2.406	0.998123529381951\\
2.409	0.997992014449511\\
2.412	0.997846733979996\\
2.415	0.997685739720462\\
2.418	0.997506729909128\\
2.421	0.99730697008977\\
2.424	0.997083192621039\\
2.427	0.996831468133259\\
2.43	0.996547039709914\\
2.433	0.99622410705605\\
2.436	0.995855542869158\\
2.439	0.995432516294623\\
2.442	0.994943987556428\\
2.445	0.994376021768134\\
2.448	0.993710845621997\\
2.451	0.992925533417149\\
2.454	0.991990151046847\\
2.457	0.990865095508578\\
2.46	0.989497222418771\\
2.463	0.987814120710641\\
2.466	0.9857155172611\\
2.469	0.983060191974643\\
2.472	0.979645853152588\\
2.475	0.975178123619241\\
2.478	0.969223525915599\\
2.481	0.96114246748493\\
2.484	0.950011215183126\\
2.487	0.934599646032506\\
2.49	0.913666514593169\\
2.493	0.887294148582087\\
2.496	0.86014681991643\\
2.499	0.843932418038141\\
2.502	0.849304297714626\\
2.505	0.872252568632172\\
2.508	0.89976486655545\\
2.511	0.923518856713455\\
2.514	0.941580906712069\\
2.517	0.954748822501754\\
2.52	0.964303425897138\\
2.523	0.971312693909095\\
2.526	0.976542119556728\\
2.529	0.980515949714241\\
2.532	0.983590374791562\\
2.535	0.986009227400828\\
2.538	0.987941773003323\\
2.541	0.989507453757076\\
2.544	0.990791988415203\\
2.547	0.991857915053892\\
2.55	0.992751578873629\\
2.553	0.993507831713853\\
2.556	0.994153241637798\\
2.559	0.994708318909089\\
2.562	0.995189083004004\\
2.565	0.995608181573951\\
2.568	0.995975700325126\\
2.571	0.996299756690868\\
2.574	0.996586940243313\\
2.577	0.996842643089416\\
2.58	0.997071310349348\\
2.583	0.997276631926832\\
2.586	0.99746169069398\\
2.589	0.997629077994192\\
2.592	0.997780984407968\\
2.595	0.99791927162879\\
2.598	0.998045529793224\\
2.601	0.998161123521954\\
};
\addplot [color=mycolor2, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
2.4	0.9979734774787\\
2.403	0.997825209814236\\
2.406	0.99766069636755\\
2.409	0.99747752421372\\
2.412	0.99727282029386\\
2.415	0.997043142962172\\
2.418	0.996784342793813\\
2.421	0.996491382387313\\
2.424	0.996158100920337\\
2.427	0.995776903479678\\
2.43	0.995338346805271\\
2.433	0.994830580685094\\
2.436	0.994238585638615\\
2.439	0.993543119246928\\
2.442	0.992719239880277\\
2.445	0.99173420838499\\
2.448	0.990544460224676\\
2.451	0.989091167286114\\
2.454	0.987293628403459\\
2.457	0.98503927422308\\
2.46	0.982168348208063\\
2.463	0.978450223811587\\
2.466	0.973546863463582\\
2.469	0.96695790326784\\
2.472	0.95794518417103\\
2.475	0.94545752569139\\
2.478	0.928169863223506\\
2.481	0.905040676268413\\
2.484	0.877332924616104\\
2.487	0.852434684174704\\
2.49	0.84364685117543\\
2.493	0.857171237082473\\
2.496	0.8835299126172\\
2.499	0.910251264862635\\
2.502	0.931805047031769\\
2.505	0.947766574259816\\
2.508	0.959316265374169\\
2.511	0.967704634034125\\
2.514	0.973886125102404\\
2.517	0.978524802220388\\
2.52	0.982071172777895\\
2.523	0.984831044611326\\
2.526	0.987014369385405\\
2.529	0.988767564824478\\
2.532	0.990194496118107\\
2.535	0.991370107954824\\
2.538	0.992349369024432\\
2.541	0.99317322236792\\
2.544	0.993872605125285\\
2.547	0.994471207054391\\
2.55	0.994987392971943\\
2.553	0.995435562542019\\
2.556	0.995827125734922\\
2.559	0.996171211946253\\
2.562	0.996475191977529\\
2.565	0.996745066792782\\
2.568	0.99698576024979\\
2.571	0.997201341804147\\
2.574	0.997395197579838\\
2.577	0.997570162971875\\
2.58	0.99772862630798\\
2.583	0.997872610535638\\
2.586	0.998003838078564\\
2.589	0.998123782696422\\
2.592	0.998233711230401\\
2.595	0.998334717420052\\
2.598	0.998427749461443\\
2.601	0.998513632592575\\
};
\end{axis}
\end{tikzpicture}%

==> Figures/RISConfiguration/name.tex <==
\newcommand{\Sub}[6]{% args: coordinate,width,length,height, color                                                                                       
                \draw[black,line width=0.2mm,fill = #6] (#1) to ($(#1)+(#2,0,0)$) to ($(#1)+(#2,0,#3)$)
                to ($(#1)+(0,0,#3)$) to (#1);
                \draw[black,line width=0.2mm,fill = #5] ($(#1)+(#2,0,0)$) to ($(#1)+(#2,0,#3)$)
                to ($(#1)+(#2,-#4,#3)$) to ($(#1)+(#2,-#4,0)$) to ($(#1)+(#2,0,0)$);
                \draw[black,line width=0.2mm,fill = #5] ($(#1)+(#2,0,#3)$) to ($(#1)+(0,0,#3)$)
                to ($(#1)+(0,-#4,#3)$) to ($(#1)+(#2,-#4,#3)$) to ($(#1)+(#2,0,#3)$);
}


\newcommand{\Patch}[5]{% args: coordinate,width,length,height, color                                                                                      
                \draw[black,line width=0.2mm] (#1) to ($(#1)+(#2,0,0)$) to ($(#1)+(#2,0,#3)$)
                to ($(#1)+(0,0,#3)$) to (#1);
                \draw[black,line width=0.2mm,fill = #5] ($(#1)+(#2,0,0)$) to ($(#1)+(#2,0,#3)$)
                to ($(#1)+(#2,-#4,#3)$) to ($(#1)+(#2,-#4,0)$) to ($(#1)+(#2,0,0)$);
                \draw[black,line width=0.2mm,fill = #5] ($(#1)+(#2,0,#3)$) to ($(#1)+(0,0,#3)$)
                to ($(#1)+(0,-#4,#3)$) to ($(#1)+(#2,-#4,#3)$) to ($(#1)+(#2,0,#3)$);
}

\newcommand{\PatchLine}[7]{% args: coordinate,width, length, height, color, Nnumber of                                elements in row, center shift on x   
                
                \node (oline) at (#1){};
               \foreach \i in {1,...,#6}
                {
                    \Patch{oline.center}{#2}{#3}{#4}{#5};
                    \node (oline) at ($(oline.center)+(#7,0,0)$) {};
                }
}

\newcommand{\diode}[5]{% args: coordinate,width,length,height, color                                                                                      
                \draw[black,line width=0.2mm,fill = #5] (#1) to ($(#1)+(#2,0,0)$) to ($(#1)+(#2,0,#3)$)
                to ($(#1)+(0,0,#3)$) to (#1);
                \draw[black,line width=0.2mm,fill = black] ($(#1)+(#2,0,0)$) to ($(#1)+(#2,0,#3)$)
                to ($(#1)+(#2,-#4,#3)$) to ($(#1)+(#2,-#4,0)$) to ($(#1)+(#2,0,0)$);
                \draw[black,line width=0.2mm,fill = #5] ($(#1)+(#2,0,#3)$) to ($(#1)+(0,0,#3)$)
                to ($(#1)+(0,-#4,#3)$) to ($(#1)+(#2,-#4,#3)$) to ($(#1)+(#2,0,#3)$);
}

\newcommand{\diodeline}[7]{% args: coordinate,width, length, height, color, Nnumber of                                elements in row, center shift on x   
                
                \node (oline) at (#1){};
               \foreach \i in {1,...,#6}
                {
                    \diode{oline.center}{#2}{#3}{#4}{#5};
                    \node (oline) at ($(oline.center)+(#7,0,0)$) {};
                }
}

\newcommand{\SurfacePatch}[9]{% args: coordinate,width, length, height, color, Nnumber of                                elements in row, center shift on x , number of rows , shift                             in row, with diode, color diode
            
            \node (o_row) at (#1){};
            \node (o_row_diode) at ($(#1)+(#2/2 -0.2/2,0, #2)$) {};            
               \foreach \i in {1,...,#8}
                {   
                % row of patches
                    \PatchLine{o_row.center}{#2}{#3}{#4}{#5}{#6}{#7};
                    \node (o_row) at ($(o_row.center)+(0,0,#9)$) {};
                    
                }

                 \foreach \i in {1,...,2}
                {   
                %row of diodes
                    
                    \diodeline{o_row_diode.center}{0.2}{0.45}{#4}{red}{#6}{#7};
                    \node (o_row_diode) at ($(o_row_diode.center)+(0,0, #9)$) {};
                    
                }

                 \node (o_feeding) at ($(#1)+(#2 + 0.7/2 - 0.2/2 ,0, 0)$) {};           
                \diodeline{o_feeding.center}{0.2}{5.5}{#4}{gray}{3}{#7};
}


\newcommand{\dogbone}[6]{% args: coordinate,width,length,height, color                                                                                      
                \draw[black,line width=0.2mm] (#1) to ($(#1)+(#2,0,0)$) to ($(#1)+(#2,0,#6)$)
                to ($(#1)+(#2/2+#6/2,0,#6)$) to ($(#1)+(#2/2+#6/2,0,#3 -#6)$) to ($(#1)+(#2,0,#3 -#6)$) to ($(#1)+(#2,0,#3)$)to ($(#1)+(0,0,#3)$)to ($(#1)+(0,0,#3 -#6)$)to ($(#1)+(#2/2-#6/2,0,#3 -#6)$)to ($(#1)+(#2/2-#6/2,0,#6)$)to ($(#1)+(0,0,#6)$) to (#1);

                 \draw[black,line width=0.2mm,fill = #5] ($(#1)+(#2,0,0)$) to ($(#1)+(#2,0,#6)$)
                to ($(#1)+(#2/2+#6/2,0,#6)$) to ($(#1)+(#2/2+#6/2,0,#3 -#6)$) to ($(#1)+(#2/2+#6/2,-#4/2,#3 -#6 - 0.1)$) to ($(#1)+(#2/2+#6/2,-#4,#6)$)to($(#1)+(#2,-#4,#6)$) to ($(#1)+(#2,-#4,0)$) to ($(#1)+(#2,0,0)$);

                \draw[black,line width=0.2mm,fill = #5]  ($(#1)+(#2,0,#3 -#6)$) to ($(#1)+(#2,0,#3)$)to ($(#1)+(0,0,#3)$) to ($(#1)+(0,-#4,#3)$) to ($(#1)+(#2,-#4,#3)$) to ($(#1)+(#2,-#4,#3 -#6)$) to ($(#1)+(#2,0,#3 -#6)$);
                }
 


 \newcommand{\DogLine}[8]{% args: coordinate,width, length, height, color, Nnumber of                                elements in row, center shift on x   
                
                \node (oline) at (#1){};
               \foreach \i in {1,...,#7}
                {
                    \dogbone{oline.center}{#2}{#3}{#4}{#5}{#6};
                    \node (oline) at ($(oline.center)+(#8,0,0)$) {};
                }
}


\newcommand{\SurfaceDog}[9]{% args: coordinate,width, length, height, color, Nnumber of                                elements in row, center shift on x , number of rows , shift                             in row, with diode, color diode
            
            \node (o_row) at (#1){};
            \node (o_row_diode) at ($(#1)+(#2/2 -0.2/2,0, #2)$) {};            
               \foreach \i in {1,...,#8}
                {   
                % row of patches
                    \DogLine{o_row.center}{#2}{#3}{#4}{#5}{0.2}{#6}{#7};
                    \node (o_row) at ($(o_row.center)+(0,0,#9)$) {};
                    
                }

                 \foreach \i in {1,...,2}
                {   
                %row of diodes
                    
                    \diodeline{o_row_diode.center}{0.2}{0.45}{#4}{red}{#6}{#7};
                    \node (o_row_diode) at ($(o_row_diode.center)+(0,0, #9)$) {};
                    
                }

                 \node (o_feeding) at ($(#1)+(#2 + 0.7/2 - 0.2/2 ,0, 0)$) {};           
                \diodeline{o_feeding.center}{0.2}{5.5}{#4}{gray}{3}{#7};
}

\definecolor{mycolor2}{rgb}{0.85000,0.500,0.09800}%



\begin{tikzpicture}

\node (o3) at (0,-3,0) {};
\Sub{o3.center}{8.5}{6.5}{.15}{black!80!green}{mycolor2};

\node (o2) at (0,-1.5,0) {};
\Sub{o2.center}{8.5}{6.5}{.3}{black!80!green}{white};
\node (oPatch) at (0.2,-1.5,0.5) {};
\SurfacePatch{oPatch.center}{1.5}{1.5}{.02}{black!60!green}{4}{2.2}{3}{2};

\node (o) at (0,0,0) {};
\Sub{o.center}{8.5}{6.5}{.3}{black!80!green}{white};
\node (oDog) at (0.2,0,0.5) {};
\SurfaceDog{oDog.center}{1.5}{1.5}{.02}{black!60!green}{4}{2.2}{3}{2};

\end{tikzpicture}

==> OldRef.tex <==
@ARTICLE{PracPhaseAmp,
  author={Li, Hongyu and Cai, Wenhao and Liu, Yang and Li, Ming and Liu, Qian and Wu, Qingqing},
  journal={IEEE Trans. on Commun.}, 
  title={Intelligent Reflecting Surface Enhanced Wideband MIMO-OFDM Communications: From Practical Model to Reflection Optimization}, 
  year={2021},
  volume={69},
  number={7},
  pages={4807-4820},
  doi={10.1109/TCOMM.2021.3069860}}

@ARTICLE{RISDesign_1,
  author={Gros, Jean-Baptiste and Popov, Vladislav and Odit, Mikhail A. and Lenets, Vladimir and Lerosey, Geoffroy},
  journal={IEEE Open Journal of the Communications Society}, 
  title={A Reconfigurable Intelligent Surface at mmWave Based on a Binary Phase Tunable Metasurface}, 
  year={2021},
  volume={2},
  number={},
  pages={1055-1064},
  doi={10.1109/OJCOMS.2021.3076271}}

  @ARTICLE{RISDesign_2,
  author={Baladi, Elham and Xu, Min Yin and Faria, Nicolas and Nicholls, Jeff and Hum, Sean Victor},
  journal={IEEE Transactions on Antennas and Propagation}, 
  title={Dual-Band Circularly Polarized Fully Reconfigurable Reflectarray Antenna for Satellite Applications in the Ku-Band}, 
  year={2021},
  volume={69},
  number={12},
  pages={8387-8396},
  doi={10.1109/TAP.2021.3090577}}


@INProc.{LargNumberOfBits,
  author={Jain, Adit and Rahul, D. and Kashyap, Salil and Sarvendranath, Rimalapudi},
  journal={2022 Nat. Conf. on Commun. (NCC)}, 
  title={Low Complexity Passive Beamforming Algorithms for Intelligent Reflecting Surfaces with Discrete Phase-Shifts over OFDM Systems}, 
  year={2022},
  volume={},
  number={},
  pages={160-165},
  doi={10.1109/NCC55593.2022.9806790}}

@INProc.{mmwave,
  author={Karjalainen, Juha and Nekovee, Maziar and Benn, Howard and Kim, Wuk and Park, JeongHo and Sungsoo, Hwang},
  booktitle={2014 9th Int.  Conf. on Cogn. Radio Oriented Wireless Networks and Commun. (CROWNCOM)}, 
  title={Challenges and opportunities of mm-wave communication in 5G networks}, 
  year={2014},
  volume={},
  number={},
  pages={372-376},
  doi={10.4108/icst.crowncom.2014.255604}}


  @INPROCEEDINGS{MIMOCom,
  author={Mohanty, Sidharth and Agarwal, Arun and Mali, Sabita and Misra, Gourav and Agarwal, Kabita},
  booktitle={2020 Fourth Int. Conf. on I-SMAC (IoT in Social, Mobile, Analytics and Cloud) (I-SMAC)}, 
  title={Design and BER Performance Analysis of MIMO and Massive MIMO Networks under Perfect and Imperfect CSI}, 
  year={2020},
  volume={},
  number={},
  pages={307-312},
  doi={10.1109/I-SMAC49090.2020.9243359}}

@ARTICLE{THzBlockedLoS,
  author={Du, Hongyang and Zhang, Jiayi and Guan, Ke and Niyato, Dusit and Jiao, Huiying and Wang, Zhiqin and Kürner, Thomas},
  journal={IEEE Trans. on Commun.}, 
  title={Performance and Optimization of Reconfigurable Intelligent Surface Aided THz Communications}, 
  year={2022},
  volume={70},
  number={5},
  pages={3575-3593},
  doi={10.1109/TCOMM.2022.3162645}}

@INProc.{PracPin,
  author={Hassouna, Saber and Rains, James and Rehman Kazim, Jalilur and Ur Rehman, Masood and Imran, Muhammad and Abbasi, Qammer H.},
  booktitle={2022 Int.  Workshop on Antenna Technol. (iWAT)}, 
  title={Discrete Phase Shifts for Intelligent Reflecting Surfaces in OFDM Communications}, 
  year={2022},
  volume={},
  number={},
  pages={128-131},
  doi={10.1109/iWAT54881.2022.9810915}}


  @book{Pozar,
      author        = "Pozar, David M",
      title         = "{Microwave engineering; 3rd ed.}",
      publisher     = "Wiley",
      address       = "Hoboken, NJ",
      year          = "2005",
      url           = "https://cds.cern.ch/record/882338",
}

@ARTICLE{AFSSResponse,
  author={Hum, Sean Victor and Perruisseau-Carrier, Julien},
  journal={IEEE Trans. on Antennas and Propagation}, 
  title={Reconfigurable Reflectarrays and Array Lenses for Dynamic Antenna Beam Control: A Review}, 
  year={2014},
  volume={62},
  number={1},
  pages={183-198},
  doi={10.1109/TAP.2013.2287296}}
  
@INProc.{PracPhaseAmp2,
  author={Abeywickrama, Samith and Zhang, Rui and Yuen, Chau},
  booktitle={ICC 2020 - 2020 IEEE Int.  Conf. on Commun. (ICC)}, 
  title={Intelligent Reflecting Surface: Practical Phase Shift Model and Beamforming Optimization}, 
  year={2020},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/ICC40277.2020.9148961}}


@ARTICLE{RISAtan,
  author={Cai, Wenhao and Li, Hongyu and Li, Ming and Liu, Qian},
 journal={IEEE Commun. Letters}, 
  title={Practical Modeling and Beamforming for Intelligent Reflecting Surface Aided Wideband Systems}, 
  year={2020},
  volume={24},
  number={7},
  pages={1568-1571},
  doi={10.1109/LCOMM.2020.2987322}}


@book{munkrequency,
title={Frequency selective surfaces: theory and design},
author={Munk, Ben A},
year={2000},
publisher={John Wiley \& Sons}
}

@ARTICLE{6gApp,
  author={Sarieddeen, Hadi and Alouini, Mohamed-Slim and Al-Naffouri, Tareq Y.},
  journal={Proc. of the IEEE}, 
  title={An Overview of Signal Processing Techniques for Terahertz Communications}, 
  year={2021},
  volume={109},
  number={10},
  pages={1628-1665},
  doi={10.1109/JPROC.2021.3100811}}

  @ARTICLE{Cluster,
  author={Liu, Yiming and Li, Xi and Yu, F. Richard and Ji, Hong and Zhang, Heli and Leung, Victor C. M.},
  journal={IEEE J. on Sel. Areas in Commun.}, 
  title={Grouping and Cooperating Among Access Points in User-Centric Ultra-Dense Networks With Non-Orthogonal Multiple Access}, 
  year={2017},
  volume={35},
  number={10},
  pages={2295-2311},
  doi={10.1109/JSAC.2017.2724680}}



@INProc.{noma,
  author={Marcano, Andrea S. and Christiansen, Henrik L.},
  booktitle={2017 Int.  Conf. on Comput., Netw. and Commun. (ICNC)}, 
  title={Performance of Non-Orthogonal Multiple Access (NOMA) in mmWave wireless Communications for 5G networks}, 
  year={2017},
  volume={},
  number={},
  pages={969-974},
  doi={10.1109/ICCNC.2017.7876265}}

@ARTICLE{usercentric,
  author={Liu, Jianghui and Zhang, Hongtao},
  journal={IEEE Wireless Commun. Letters}, 
  title={Power Allocation in Ultra-Dense Networks Through Deep Deterministic Policy Gradient}, 
  year={2022},
  volume={11},
  number={12},
  pages={2502-2506},
  doi={10.1109/LWC.2022.3206096}}



  
  

  @ARTICLE{machinedense,
  author={Liao, Wei-Shun and Zhao, Ou and Kibria, Mirza Golam and Villardi, Gabriel Porto and Ishizu, Kentaro and Kojima, Fumihide},
  journal={IEEE Access}, 
  title={Machine Learning-Based Signal Detection for CoMP Downlink in Ultra-Dense Small Cell Networks}, 
  year={2020},
  volume={8},
  number={},
  pages={17454-17463},
  doi={10.1109/ACCESS.2020.2965631}}

  @INProc.{extradens,
  author={Lai, Wei Kuang and Hsu, Chia-Yu and Kuo, Yu-Po},
  booktitle={2019 20th Asia-Pacific Network Operations and Manage. Symp. (APNOMS)}, 
  title={QoS-guaranteed User Association and Resource Allocation with CoMP JT in Ultra-Dense Networks}, 
  year={2019},
  volume={},
  number={},
  pages={1-6},
  doi={10.23919/APNOMS.2019.8892951}}

@INProc.{Relay,
  author={Padhy, Saraju Prasad and Sethi, Srinivas and Tripathy, Aruna},
  booktitle={2018 Int.  Conf. on Appl. Electromagnetics, Signal Process. and Communication (AESPC)}, 
  title={Performance evaluation of Relays used for next Generation wireless communication networks}, 
  year={2018},
  volume={1},
  number={},
  pages={1-4},
  doi={10.1109/AESPC44649.2018.9033327}}


  @ARTICLE{RISoverview,
  author={Jian, Mengnan and Alexandropoulos, George C. and Basar, Ertugrul and Huang, Chongwen and Liu, Ruiqi and Liu, Yuanwei and Yuen, Chau},
  journal={Intell. and Converged Networks}, 
  title={Reconfigurable intelligent surfaces for wireless Communications: Overview of hardware designs, channel models, and estimation techniques}, 
  year={2022},
  volume={3},
  number={1},
  pages={1-32},
  doi={10.23919/ICN.2022.0005}}

  @ARTICLE{RISPro,
  author={Fara, Roman and Ratajczak, Philippe and Phan-Huy, Dinh-Thuy and Ourir, Abdelwaheb and Di Renzo, Marco and de Rosny, Julien},
  journal={IEEE Wireless Commun.}, 
  title={A Prototype of Reconfigurable Intelligent Surface with Continuous Control of the Reflection Phase}, 
  year={2022},
  volume={29},
  number={1},
  pages={70-77},
  doi={10.1109/MWC.007.00345}}

  @ARTICLE{amplifierRIS,
  author={Khoshafa, Majid H. and Ngatched, Telex M. N. and Ahmed, Mohamed H. and Ndjiongue, Alain R.},
  Converged={IEEE Commun. Letters}, 
  title={Active Reconfigurable Intelligent Surfaces-Aided Wireless Communication System}, 
  year={2021},
  volume={25},
  number={11},
  pages={3699-3703},
  doi={10.1109/LCOMM.2021.3110714}}

  @INProc.{RISPolar,
  author={Zhang, Yunxiang and Zhao, Zhiqin and Wu, Jiangniu and Lv, Bo},
  booktitle={Proc. of 2014 3rd Asia-Pacific Conf. on Antennas and Propagation}, 
  title={A new sandwich linear polarization and frequency selective surface design}, 
  year={2014},
  volume={},
  number={},
  pages={940-942},
  doi={10.1109/APCAP.2014.6992657}}

  @ARTICLE{MISORIS,
  author={Nadeem, Qurrat-Ul-Ain and Kammoun, Abla and Chaaban, Anas and Debbah, Mérouane and Alouini, Mohamed-Slim},
  journal={IEEE Trans. on Wireless Commun.}, 
  title={Asymptotic Max-Min SINR Analysis of Reconfigurable Intelligent Surface Assisted MISO Systems}, 
  year={2020},
  volume={19},
  number={12},
  pages={7748-7764},
  doi={10.1109/TWC.2020.2986438}}

  @INProc.{MIMORIS,
  author={Ardah, Khaled and Gherekhloo, Sepideh and de Almeida, André L. F. and Haardt, Martin},
  booktitle={ICASSP 2022 - 2022 IEEE Int.  Conf. on Acoust., Speech and Signal Process. (ICASSP)}, 
  title={Double-RIS Versus Single-RIS Aided Systems: Tensor-Based Mimo Channel Estimation and Design Perspectives}, 
  year={2022},
  volume={},
  number={},
  pages={5183-5187},
  doi={10.1109/ICASSP43922.2022.9746287}}

  @ARTICLE{NOMARIS,
  author={Zhao, Boqun and Zhang, Chao and Yi, Wenqiang and Liu, Yuanwei},
  journal={IEEE Commun. Letters}, 
  title={Ergodic Rate Analysis of STAR-RIS Aided NOMA Systems}, 
  year={2022},
  volume={26},
  number={10},
  pages={2297-2301},
  doi={10.1109/LCOMM.2022.3194363}}

  @INProc.{IRSOFDM,
  author={Jiang, Weiheng and Chen, Bolin and Garg, Sahil and Nie, Jiangtian and Zhao, Jun and Xiong, Zehui},
  booktitle={2021 IEEE Global Commun. Conf. (GLOBECOM)}, 
  title={Joint Transmit Precoding and Reflect Beamforming for IRS-Assisted MIMO-OFDM Secure Communications}, 
  year={2021},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/GLOBECOM46510.2021.9685734}}

  @INProc.{RISstableband,
  author = {Alexandropoulos, George and Phan-Huy, Dinh-Thuy and Katsanos, Kostantinos and Crozzoli, Maurizio and Wymeersch, Henk and Popovski, Petar and Ratajczak, Philippe and Bénédic, Yohann and Hamon, Marie-Helene and Gonzalez, Sebastien and Mursia, Placido and Rossanese, Marco and Sciancalepore, Vincenzo and Gros, Jean-Baptiste and Terranova, Sergio and Gradoni, Gabriele and Di Lorenzo, Paolo and Rahal, Moustafa and Denis, Benoit and Strinati, Emilio},
year = {2023},
month = {03},
pages = {},
title = {RIS-Enabled Smart Wireless Environments: Deployment Scenarios, Network Architecture, Bandwidth and Area of Influence}
}

  @ARTICLE{RISLoc,
  author={Lin, Yuxing and Jin, Shi and Matthaiou, Michail and You, Xiaohu},
  journal={IEEE Trans. on Wireless Commun.}, 
  title={Channel Estimation and User Localization for IRS-Assisted MIMO-OFDM Systems}, 
  year={2022},
  volume={21},
  number={4},
  pages={2320-2335},
  doi={10.1109/TWC.2021.3111176}}

  @INProc.{CSIOne,
  author={Mishra, Deepak and Johansson, Håkan},
  booktitle={ICASSP 2019 - 2019 IEEE Int.  Conf. on Acoust., Speech and Signal Process. (ICASSP)}, 
  title={Channel Estimation and Low-complexity Beamforming Design for Passive Intelligent Surface Assisted MISO Wireless Energy Transfer}, 
  year={2019},
  volume={},
  number={},
  pages={4659-4663},
  doi={10.1109/ICASSP.2019.8683663}}

  @ARTICLE{CSIML,
  author={Taha, Abdelrahman and Alrabeiah, Muhammad and Alkhateeb, Ahmed},
  journal={IEEE Access}, 
  title={Enabling Large Intelligent Surfaces With Compressive Sensing and Deep Learning}, 
  year={2021},
  volume={9},
  number={},
  pages={44304-44321},
  doi={10.1109/ACCESS.2021.3064073}}


  @inProc.{RicianChannel,
  title={On the capacity of MIMO rice channels},
  author={Laura Cottatellucci},
  year={2004}
}

@INProc.{LoCOFDMIdeal,
  author={He, Jiguang and Wymeersch, Henk and Kong, Long and Silvén, Olli and Juntti, Markku},
  booktitle={2020 IEEE 91st Veh. Technol. Conf. (VTC2020-Spring)}, 
  title={Large Intelligent Surface for Positioning in Millimeter Wave MIMO Systems}, 
  year={2020},
  volume={},
  number={},
  pages={1-5},
  doi={10.1109/VTC2020-Spring48590.2020.9129075}}


@ARTICLE{waterfilling,
  author={He, Peter and Zhao, Lian and Zhou, Sheng and Niu, Zhisheng},
  J.={IEEE Trans. on Wireless Commun.}, 
  title={Water-Filling: A Geometric Approach and its Application to Solve Generalized Radio Resource Allocation Problems}, 
  year={2013},
  volume={12},
  number={7},
  pages={3637-3647},
  doi={10.1109/TWC.2013.061713.130278}}

  @ARTICLE{APHPBWNour,
  author={Kouzayha, Nour and Kishk, Mustafa A. and Sarieddeen, Hadi and Alouini, Mohamed-Slim and Al-Naffouri, Tareq Y.},
  journal={IEEE Trans. on Wireless Commun.}, 
  title={Coexisting Terahertz and RF Finite Wireless Networks: Coverage and Rate Analysis}, 
  year={2022},
  volume={},
  number={},
  pages={1-1},
  doi={10.1109/TWC.2022.3229745}}

  @ARTICLE{QOSIRS,
  author={Cai, Yuanxin and Wei, Zhiqiang and Hu, Shaokang and Liu, Chang and Ng, Derrick Wing Kwan and Yuan, Jinhong},
  J.={IEEE Trans. on Wireless Commun.}, 
  title={Resource Allocation and 3D Trajectory Design for Power-Efficient IRS-Assisted UAV-NOMA Communications}, 
  year={2022},
  volume={21},
  number={12},
  pages={10315-10334},
  doi={10.1109/TWC.2022.3183300}}

  @INProc.{QOSMIMO,
  author={de Pinho, Carlos Augusto Melo and Lima, Francisco Rafael Marques},
  journal={2022 Workshop on Communication Networks and Power Syst. (WCNPS)}, 
  title={Rate maximization with QoS guarantees in IRS-assisted WPCN-NOMA systems}, 
  year={2022},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/WCNPS56355.2022.9969722}}


  @ARTICLE{EqualPA,
  author={Lin, Shaoe and Zheng, Beixiong and Alexandropoulos, George C. and Wen, Miaowen and Chen, Fangjiong and sMumtaz, Shahid},
  journal={IEEE J. on Sel. Areas in Commun.}, 
  title={Adaptive Transmission for Reconfigurable Intelligent Surface-Assisted OFDM Wireless Communications}, 
  year={2020},
  volume={38},
  number={11},
  pages={2653-2665},
  doi={10.1109/JSAC.2020.3007038}}

    @ARTICLE{MaxRatTRan,
  author={Lo, T.K.Y.},
  journal={IEEE Trans. on Commun.}, 
  title={Maximum ratio transmission}, 
  year={1999},
  volume={47},
  number={10},
  pages={1458-1461},
  doi={10.1109/26.795811}}

  @ARTICLE{ZeroForcing,
  author={Liu, Guangyi and Bala, Erdem and Li, Lu and Cimini, Leonard J.},
  journal={IEEE Trans. on Veh. Technol.}, 
  title={Outage Analysis for MISO Zero-Forcing Precoding With Outdated CSI}, 
  year={2020},
  volume={69},
  number={8},
  pages={9152-9156},
  doi={10.1109/TVT.2020.2999512}}

  @INProc.{PlannerWave,
  author={Amar, A. and Weiss, A.J.},
  booktitle={2004 IEEE Int.  Conf. on Acoust., Speech, and Signal Process.}, 
  title={Direct position determination of multiple radio signals}, 
  year={2004},
  volume={2},
  number={},
  pages={ii-81},
  doi={10.1109/ICASSP.2004.1326199}}

  @INProc.{LocIdeal,
  author={Fascista, Alessio and Coluccia, Angelo and Wymeersch, Henk and Seco-Granados, Gonzalo},
  booktitle={ICASSP 2021 - 2021 IEEE Int.  Conf. on Acoust., Speech and Signal Process. (ICASSP)}, 
  title={RIS-Aided Joint Localization and Synchronization with a Single-Antenna Mmwave Receiver}, 
  year={2021},
  volume={},
  number={},
  pages={4455-4459},
  doi={10.1109/ICASSP39728.2021.9413515}}
